Collaborative Behavior Models for Optimized Human-Robot Teamwork

Effective human-robot collaboration requires informed anticipation. The robot must anticipate the human's actions, but also react quickly and intuitively when its predictions are wrong. The robot must plan its actions to account for the human's own plan, with the knowledge that the human's behavior will change based on what the robot actually does. This cyclical game of predicting a human's future actions and generating a corresponding motion plan is extremely difficult to model using standard techniques. In this work, we describe a novel Model Predictive Control (MPC)-based framework for finding optimal trajectories in a collaborative, multi-agent setting, in which we simultaneously plan for the robot while predicting the actions of its external collaborators. We use human-robot handovers to demonstrate that with a strong model of the collaborator, our framework produces fluid, reactive human-robot interactions in novel, cluttered environments. Our method efficiently generates coordinated trajectories, and achieves a high success rate in handover, even in the presence of significant sensor noise.

==> Old Sections/04Outline.tex <==

Our key contributions are
%\begin{itemize}
    %\item 
    (1) A framework for jointly optimizing a robot's actions and predicting human behavior assuming cooperative intent in a single optimization process.
    %\item 
    (2) A sparse reward framework for attaining spatial consistency of a continuously running finite-horizon MPC optimization process, enabling behavioral consistency across re-plans.
    %\item 
    (3) The use of this MPC process as a reactive MAP belief-space approximate POMDP solver \cite{MurphyPOMDPSolvers2000} to accommodate the inherent uncertainty in the uncontrolled predictions of the human's behavior.
    
In section \ref{}, we will lay out a general optimization framework for human-robot collaboration. 
We demonstrate the framework on the problem in human-robot handover in section \ref{}. 
Then, in section \ref{}, we evaluate our method against several other methods for human-robot handovers and demonstrate its robustness to sensor noise.
See our video submission for additional videos of our experiments.

==> Old Sections/05human.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.49\columnwidth}
    \centering
    \raisebox{2.8ex}{
        \includegraphics[width=.9\columnwidth]{Figures/reach_to_point_setup.pdf}
    }
    \caption{A reach-to-point task around an obstacle}
\end{subfigure}
\begin{subfigure}[t]{0.49\columnwidth}
    \centering
    \includegraphics[width=.9\columnwidth]{Figures/3D/3D_human_eval.png}
    \caption{An example of our prediction aligned with the human's true trajectory}
\end{subfigure}
\caption{We recorded 29 trials of a reach-to-point task, with varying target points, camera poses, and starting positions. We used 26 datasets to tune the model and 3 datasets to evaluate.}
\label{fig:human-prediction}
\end{figure}
Our model for optimal human reaching, as described in section \ref{sec:human}, is a parametrized quadratic cost function symmetrical to the robot. To evaluate our model, we recorded 29 reach-to-point tasks around an obstacle using the Microsoft Azure Kinect. Between trials, we randomly changed the target position, the human's starting pose, and the camera height. 

In our experimental setup, we observed that the Azure's estimate of the target pose, which we tracked using ALVAR \footnote{\url{https://wiki.ros.org/ar_track_alvar}}, is very stable.
In each dataset, we measured the the distances from each target position estimate to the mean target position. We then averaged this number over our 29 datasets to get a mean target estimator error of $0.13$cm. 

We also sought to evaluate the stability of the Azure Body Tracking SDK. In each trial, we know the human touches the target, so the distance from the fingertip estimate and the target pose when the human touches it can serve as a proxy for measurement error. Over our dataset, we found this error to $3.28$cm, with a standard deviation of $3.68$cm. 

Over the entire reach-to-point action, we measured pose estimation error as the shortest distance between the fingertip pose estimates and the mean target pose. Over all  target and the hand pose estimate from the Azure Body Tracking SDK over the entire trajectory. error in the Azure's tracking of the target pose to be 

For each trial, we calculated our prediction error with 
\begin{eqnarray}
\text{Loss} = \sum_{t = 0}^{T}\frac{1}{T - (t + 1)} \sum_{i=t + 1}^{T}\norm{x_{\text{predicted}} - x_{\text{measured}}}^2
\end{eqnarray}
where $T$ is the total number of time steps it takes the human to reach the target and $x$ is the position of the hand. This loss represents the average distance between the corresponding real and predicted hand poses, which we then average over all MPC steps. We used $26$ of our trials to tune our human model and performed a grid search over $6,561$ parameter configurations to minimize error. We then evaluated the parameters on the remaining $3$ datasets. Our average loss on the training set $7.54$cm and our average loss on the evaluation set is $9.63$cm.

